Small Cuts and Connectivity Certificates: A Fault Tolerant Approach

We revisit classical connectivity problems in the CONGEST model of distributed computing. By using techniques from fault tolerant network design, we show improved constructions, some of which are even "local" (i.e., with $\widetilde{O}(1)$ rounds) for problems that are closely related to hard global problems (i.e., with a lower bound of $\Omega(Diam+\sqrt{n})$ rounds). Our main results are: (1) For $D$-diameter unweighted graphs with constant edge connectivity, we show an exact distributed deterministic computation of the minimum cut in $poly(D)$ rounds. This resolves one the open problems recently raised in Daga, Henzinger, Nanongkai and Saranurak, STOC'19. (2) For $D$-diameter unweighted graphs, we present a deterministic algorithm that computes of all edge connectivities up to constant in $poly(D)\cdot 2^{O(\sqrt{\log n\log\log n})}$ rounds. (3) Computation of sparse $\lambda$ connectivity certificates in $\widetilde{O}(\lambda)$ rounds. Previous constructions where known only for $\lambda \leq 3$ and required $O(D)$ rounds. This resolves the problem raised by Dori PODC'18.

==> minimum-cuts-new-new.tex <==
\vspace{-15pt}\section{Exact Computation of Small Cuts} %\vspace{-10pt}
Throughout, we consider unweighted multigraphs with diameter $D$, and (edge or vertex) connectivity at most $\lambda=O(1)$. Before presenting the algorithm we start by considering the following  simpler task.
%We will first describe the randomized algorithm for computing the exact minimum edge cuts. Similar algorithm applies also for vertex cuts (but with somewhat worse bounds). 
%Before presenting the minimum cut algorithm, we start by introduce the notion $(s,t)$ connectivity certificates, which play a key role in our minimum cut computation.
%\dnsparagraph{$(s,t)$ connectivity certificates}

%For every pair of vertices $s$ and $t$, the $(s,t)$\emph{connectivity certificate} is a subgraph $G_{s,t} \subseteq G$ satisfying that $s$ and $t$ are $\lambda$ connected in $G$ iff then they are also $\lambda$-connected in $G_{s,t}$. Whereas a-priori the size of the subgraph $G_{s,t}$ (number of edges) might be large, we bound it as a function of the graph diameter $D$ and $\lambda$. \vspace{-3pt}
%\begin{lemma}
%Fix a connectivity value $\lambda$ and a source vertex $s$. Then $|G_{s,t}|=O(D^{\lambda})$ for every $t \in V$, and this is \emph{tight} (see Fig. \ref{fig:st-certificate}). 
%\end{lemma} \vspace{-3pt}
%Having this bound is still insufficient, as we will need to compute the $(s,t)$ connectivity certificate for every $t \in V$. By using the FT-sampling approach (described next), we compute these $n-1$ certificates simultaneously, in almost linear time in the \emph{size} of the individual certificate. This immediately leads to a minimum cut computation, as there must be a vertex $t$ which is separated from $s$ by the edges of the minimum cut.
\dnsparagraph{Warm Up: Cut Verification}
%The key lemma for showing that such certificates have small size and can be computed efficiently is the following: 
In the cut verification problem, one is given a subset of edges $E'$ where $|E'|\leq \lambda$, it is then required to test if $G \setminus E'$ is connected. As we will see there is a simple algorithm for this problem which is based on the following key lemma.
\vspace{-5pt}
\begin{lemma}\label{lem:bounded-length-connected}
Consider a $D$-diameter unweighted graph $G=(V,E)$ with maximum degree $\Delta$. 
(1) If $u,v \in V$ are $\lambda$-edge connected\footnote{Note that we do not require the graph $G$ to be $\lambda$ connected.} (i.e., the $u$-$v$ cut is at least $\lambda$) then $\dist(u,v, G \setminus F)\leq c\cdot\lambda \cdot D$ for every edge sequence $F \subseteq E$, $|F|\leq \lambda-1$ for some constant $c$. \\
(2) If $u,v \in V$ are $\lambda$-vertex connected then $\dist(u,v, G \setminus F)\leq c \cdot \lambda \cdot\Delta \cdot D$ for every vertex sequence $F \subseteq V$, $|F|\leq \lambda-1$. 
\end{lemma}%\vspace{-5pt}
%\def\APPENDBOUNDEDLC{
\begin{proof}%[Proof of Lemma \ref{lem:bounded-length-connected}]
Let $T$ be an arbitrary BFS tree in $G$ of diameter $O(D)$. We begin with (1). Fix a set of faults $F \subseteq E$, $|F| \leq \lambda-1$, and let $P_{u,v,F}$ be the $u$-$v$ shortest path in $G \setminus F$. Since $u$ and $v$ are $\lambda$-edge connected such path $P_{u,v,F}$ exists. We next bound the length of $P_{u,v,F}$. Consider the forest $T \setminus F$ which has at most $\lambda$ connected components $C_1,\ldots, C_\ell$. We mark each vertex on $P_{u,v,F}$ with its component ID in the forest $T \setminus F$. Note that all vertices in the same component are connected by a path of length $O(D)$ in $G \setminus F$. We can then traverse the path $P_{u,v,F}$ from $u$ and jump to the last vertex $u_1$ on the path (close-most to $v$) that belongs to the component of $u$. The length of this sub-path is $O(D)$ and using one connecting edge on $P_{u,v,F}$, we move to a vertex belonging to a new component in $T \setminus F$. Overall the path $P_{u,v,F}$ can be covered by $\lambda$ path segments $P_1,\ldots, P_{\ell}$ such that the endpoints of each segments are in the \emph{same} component in $T \setminus F$, each neighboring segments $P_i$ and $P_{i+1}$ are connected by an edge from $P_{u,v,F}$. Since each $|P_i|=O(D)$, we get that $|P_{u,v,F}|=O(\lambda \cdot D)$. 
Claim (2) follows the exact same argument with the only distinction is that when a vertex fails, the BFS tree might break up into $\Delta+1$ components. Thus, for a subset $F \subseteq V$ of vertices with $|F|\leq \lambda-1$, the tree $T$ breaks into $O(\lambda \cdot \Delta)$ components.
\end{proof}
%}%\APPENDBOUNDEDLC
This lemma immediately implies an $O(\lambda D)$-round solution for the cut verification task: build a BFS tree $T$ from an arbitrary source up to depth $O(\lambda \cdot D)$. Then $T$ is a spanning tree iff $E'$ does not disconnect the graph. \vspace{-7pt}
\begin{corollary}\label{cor:cut-verification}[Cut Verification]
Given a set of $\lambda$ edges $E'$. One can test if $E'$ is a cut in $G$ using $O(\lambda \cdot D)$ rounds. 
%(and this is tight\footnote{It is easy to show that there are $D$-diameter and $\lambda$ connected graphs for which a removal of $\lambda-1$ edges increases the diameter by a of factor $\Omega(\lambda)$.}).
\end{corollary}

%
%
%
%
%
%The algorithm is based on Lemma \ref{lem:bounded-length-connected} and a sampling technique borrowed from fault tolerant network design \cite{weimann2013replacement,dinitz2011fault}.
%The randomized algorithm for minimum cut is based on computing the $(s,t)$ connectivity certificate $G_{s,t}\subset G$ for every $t \in V$ given a fixed source $s$. 
The following definition is useful for the description and analysis of our algorithm.
\begin{definition}[$(s,t)$ connectivity certificate]
Given a graph $G$ with minimum cut $\lambda$ and a pair of vertices $s$ and $t$, the $(s,t)$ \emph{connectivity certificate} is a subgraph $G_{s,t} \subseteq G$ satisfying that $s$ and $t$ are $\lambda$-connected in $G_{s,t}$ iff they are $\lambda$-connected in $G$.
\end{definition}\vspace{-7pt}
Whereas a-priori the size of the $s$-$t$ connectivity certificate, measured by the number of edges, might be $\Omega(n)$, as will show later on, it is in fact bounded by $(\lambda D)^{O(\lambda)}$, hence $\poly(D)$ for $\lambda=O(1)$. With this definition in mind, we are now ready to present the minimum cut algorithm.

\paragraph{A $\poly(D)$-Round Randomized Algorithm.}
The algorithm has two phases. In the first phase, every vertex $t$ computes its $(s,t)$ certificate subgraph $G_{s,t}$ w.r.t. a given fixed source $s$. In the second phase, each vertex $y$ locally computes its $s$-$t$ cut in the subgraph $G_{s,t}$, and one of the output $\lambda$-size cut is broadcast to the entire network. 
%
%We now focus on the first phase. In the second phase, every vertex $v$ locally computes its minimum $s$-$v$ cut in the subgraph $E_v$. 
Throughout, we assume w.l.o.g. that the value of the minimum cut $\lambda$ is known, since $\lambda=O(1)$ this assumption can be easily removed.

The first phase has $\ell=O((\lambda D)^{2\lambda})$ iterations, or \emph{experiments}. 
In each iteration $i$, the algorithm samples a subgraph $G_i$ by including each edge $e \in G$ into $G_i$ independently with probability $p=1-1/(c(\lambda D))$ for some constant $c$ 
(taken from Lemma \ref{lem:bounded-length-connected}). 
For a source vertex $s$ (which is fixed in all iterations), a (truncated) BFS tree $B_i$ rooted in $s$ is computed in $G_i$ up to depth $c\cdot \lambda \cdot D$.
Next, every vertex in $B_i$ learns its tree path from $s$ by pipelining these edges downward the tree. This completes the description of an iteration. Let $G_{s,t}=\bigcup_{i=1}^{\ell} \pi(s,t,B_i)$.

%At the end of these $\ell$ iterations, each vertex locally computes its $s$-$v$ connectivity in the graph 
In the second phase, every vertex $t$ locally computes its $s$-$t$ cut in the subgraph $G_{s,t}$.
The edges of the minimum cut are those obtained by one of the vertices $t$ whose $s$-$t$ connectivity in $G_{s,t}$ is at most $\lambda$. 

\dnsparagraph{Correctness} 
%Since each $G_{s,t} \subseteq G$, clearly there exists at least one vertex $t$ with $\lambda(s,t,G_{s,t})\leq\lambda$ (I.e., the vertex that does not belong to the component of $s$ in $G \setminus E^*$ where $E^*$ is one of the minimum cuts in $G$). Thus, it is sufficient to show that w.h.p. every vertex $t$ with $\lambda(s,t,G_{s,t})\leq\lambda$ outputs a legal minimum cut.
For the correctness of the algorithm it will be sufficient to show that w.h.p. $G_{s,t}$ is an $s$-$t$ connectivity certificate for every $t \in V$.
%, by showing that for every subset $F \subseteq G$ of at most $\lambda$ edge faults, $s$ and $t$ are connected in $G\setminus F$ iff they are connected in $G_{s,t}\setminus F$. 
%Consider a vertex $v$ with $\lambda(s,v,G_v)\leq\lambda$ and let $E'$ be the $s$-$v$ cut in $E_v$. We will claim that w.h.p. $E_v$ is also cut in $G$ by showing that $s$ and $v$ are not connected in $G \setminus E'$. 
\begin{claim}\label{cl:succprobcut}
For every $t$, w.h.p., $G_{s,t}$ is an $s$-$t$ connectivity certificate.
% that is for every triplet $\langle s,t,F \rangle$ for $|F|\leq \lambda$, $s$ and $t$ are connected in $G_{s,t} \setminus F$, iff they are also connected in $G\setminus F$. 
\end{claim}
%\def\APPENDCLSUCCEXP{
\begin{proof}%[Proof of Cl. \ref{cl:succprobcut}]
Since $G_{s,t} \subseteq G$, it is sufficient to show that $s$ and $t$ are connected in $G_{s,t} \setminus F$ for any subset $F \subset E$, $|F|\leq \lambda$ satisfying that $s$ and $t$ are connected in $G \setminus F$. 
Fix such a triplet $\langle s,t,F \rangle$ where $s$ and $t$ are connected in $G \setminus F$. 
%(Since $G_{s,t} \subseteq G$, this is the only interesting case).  
An iteration $i$ is \emph{successful} for $\langle s,t, F \rangle$ if 
$$\pi(s,t,G\setminus F)\subseteq G_i \mbox{~~and~~} F \cap G_i=\emptyset.$$
Note that if iteration $i$ is successful for $\langle s,t, F \rangle$, then the truncated BFS tree $B_i$ contains $t$ as $\dist(s,t,G_i)= |\pi(s,t,G\setminus F)|\leq c\cdot \lambda \cdot D$, where the last inequality is due to Lemma \ref{lem:bounded-length-connected}(1). In addition, since $F \cap G_i=\emptyset$, it also holds that $\pi(s,t,B_i)\subseteq G_{s,t} \setminus F$.

It remains to show that with probability at least $1-1/n^{\Omega(\lambda)}$, every triplet $\langle s,t, F \rangle$ where $s$ and $t$ are connected in $G \setminus F$, has at least one successful iteration. The claim will then follow by applying the union bound over all $n^{2\lambda}$ triplets. Recall that each edge is sampled into $G_i$ independently with probability $p$. Thus the probability that iteration $i$ is successful for $\langle s,t, F \rangle$ is at least: 
$$q=p^{(c\cdot \lambda D)}\cdot (1-p)^\lambda=1/(\lambda\cdot D)^{\lambda}.$$ 
Since there are $\ell$ independent experiments, the probability that all of them fail is $(1-q)^{\ell}\leq 1/n^{\Omega(\lambda)}$, the claim follows.
\end{proof}
%}%\APPENDCLSUCCEXP
%\APPENDCLSUCCEXP
Finally, let $t$ be a vertex such that $s$ and $t$ are not $(\lambda+1)$-connected in $G$. Thus, by the lemma above, $\lambda(s,t,G_{s,t})\leq \lambda$ and the minimum cut computation applied locally by vertex $t$ in $G_{s,t}$ outputs a subset $F$ of at most $\lambda$ edges. We claim that w.h.p. $s$ and $t$ are also not connected in $G \setminus F$. Assume otherwise, then by Lemma \ref{lem:bounded-length-connected}(1),  $\dist(s,t,G \setminus F)\leq c\cdot \lambda \cdot D$, thus by the argument above, w.h.p., there is an iteration $i$ in which an $s$-$t$ path that does not go through $F$ is taken into $G_{s,t}$, leading to a contradiction that $s$ and $t$ are disconnected in $G_{s,t}\setminus F$.  

%
%$E_{s,t}$, $|F|\leq \lambda-1$, such that $s$ and $t$ are not connected in $G_{s,t} \setminus F$, then w.h.p. they are also not connected in $G$. This established the correctness of the computed minimum cut. 
\vspace{-7pt}
\begin{corollary}
For every $D$-diameter unweighted graph $G=(V,E)$, $\lambda\geq 1$ and vertex pair $s,t \in V$, there exists an $(s,t)$ certificate $G_{s,t} \subseteq G$ of size $(\lambda D)^{O(\lambda)}$.
%, and this is existentially tight (see Fig. \ref{fig:st-certificate}).
\end{corollary}\vspace{-7pt}
\def\APPENDFIGCERT{
\begin{figure} 
	\begin{center}
		\includegraphics[scale=0.4]{st-certificate.pdf}
	\end{center}
	\caption{An illustration of $s$-$t$ certificate of size $\Omega(D^{\lambda})$. Shown is a pair of neighbors $s$ and $t$. Every edge in this graph lies on a cycle of length $\Theta(D)$. Thus, the removal, of each edge increases the length of the given shortest-path by an additive factor of $D$. Note that in this example, $\dist(s,t, G \setminus F)=\Theta(D \cdot \lambda)$ for every $|F|\leq \lambda$. However, in the collection of $\lambda$-edge disjoint $s$-$t$ paths the length of each path is $\Theta(D^{\lambda})$. The sparse certificate $G_{s,t} \subseteq G$ of $s$ and $t$ must include all those edges, leading to the size bound of $D^{O(\lambda})$ edges.}
\end{figure} \label{fig:st-certificate}
}%\APPENDFIGCERT{

\dnsparagraph{Round Complexity} Each of the $\ell$ iterations takes $O(\lambda \cdot D)$ rounds for computing the truncated BFS tree. Learning the edges along the tree path from the root also takes $O(\lambda \cdot D)$ rounds via pipeline, thus overall the round complexity is $(\lambda \cdot D)^{(c+2)\lambda}=\poly(D)$ for $\lambda=O(1)$. 

\dnsparagraph{Extension to Vertex Cuts} The algorithm for computing vertex cuts is almost identical and requires  minor adaptations. First, instead of having a single source vertex $s$, we will pick $\lambda+1$ arbitrary sources $s_1,\ldots, s_{\lambda+1}$ and will run an algorithm, which is very similar to the one described above, with respect to each source $s_i$. Note that since the vertex cut has size $\lambda$, then there is at least one vertex cut $V' \subset V$ of size $\lambda$ that does not contain at least one of the sources $s_i$. In such a case, our algorithm will find the cut $V'$ when running the below mentioned algorithm w.r.t the source $s_i$. 

The algorithm for each source $s_i$ works in iterations, where each iteration $j$ samples into a subgraph $G_j$ a collection of vertices rather than edges. That is, the subgraph $G_j$ is defined by taking the induced graph on a sample of vertices, where each vertex gets sampled independently with probability 
$p'=(1-1/(c\lambda \cdot \Delta \cdot D))$ (the constant $c$ is taken from Lemma \ref{lem:bounded-length-connected}(2)). Then a BFS tree $B_j$ rooted at $s_i$ is computed in $G_j$ up to depth $c\lambda \cdot \Delta \cdot D$. Every vertex $v \in B_j$ collects its path from the root. Let $G_{s_i,t}$ be the union of all paths collected for each vertex $t$. In the second phase, the vertex $t$ computes locally the $s_i$-$t$ vertex-cut in $G_{s_i,t}$. The analysis is then identical to that of the edge case, where in particular, we get that w.h.p. $G_{s_i,t}$ is the vertex-connectivity certificate for every $t$. 


%The deterministic computation of min-cut via derandomization of the FT-sampling (Thm. \ref{thm:min-cut-det}) appears in Appendix \ref{sec:det-cut}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% append%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-10pt}
\subsection{Deterministic Min-Cut Algorithms via Universal Sets}\label{sec:det-cut}\vspace{-5pt}
Our goal in this section is to derandomize the FT-sampling technique by locally computing explicitly (at each node) a \emph{small} family of graphs $\mathcal{G}=\{G_i \subseteq G\}$ such that in iteration $i$, the vertices will apply the computation on the graph $G_i$ in the same manner as in the randomized algorithm. Here, however, the graph $G_i$ is not sampled but rather computed locally by all the vertices. The family of subgraphs $\mathcal{G}$ is required to satisfy the following crucial property for $a=c \cdot D \cdot \lambda$ and $b=\lambda$:
\begin{mdframed}[hidealllines=false,backgroundcolor=white!25]
For every two disjoint subsets of edges $A,B$ with $|A|\leq a$ and $|B|\leq b$, there exists a subgraph $G_i \in \mathcal{G}$ satisfying that:
\begin{equation}\label{eq:det-sample}
A \subseteq G_i\mbox{~~and~~} B \cap G_i=\emptyset~.
\end{equation}
\end{mdframed}
\vspace{-5pt} In our algorithms, the subset $B$ corresponds to a set of edge faults, and $A$ corresponds to an $s$-$t$ shortest path in $G \setminus B$. Thus, $|B| \leq \lambda$ and by Lemma \ref{lem:bounded-length-connected}, $|A|=O(\lambda \cdot D)$. 
We begin with the following observation that follows by the probabilistic method.
%\vspace{-7pt}
\begin{lemma}\label{lem:prob-approach-det-sample}
There exists a family of graphs $\mathcal{G}=\{G_i \subseteq G\}$ of size $O(a^{b+1}\cdot \log n)$ that satisfies Eq. (\ref{eq:det-sample}) for every disjoint $A,B\subseteq E$ with $|A|\leq a$ and $|B|\leq b$. 
\end{lemma}%\vspace{-7pt}
%\def\APPENDLEMPROB{
\begin{proof}%[Proof of Lemma \ref{lem:prob-approach-det-sample}]
We will show that a random family $\mathcal{G}_R$ with $\ell=O(a^{b+1}\cdot \log n)$ subgraphs satisfies Eq. (\ref{eq:det-sample}) with non-zero probability. Each subgraph $G_i$ in $\mathcal{G}_R$ is computed by sampling each edge in $G$ into $G_i$ with probability of $p=(1-1/a)$. 

The probability that $G_i$ satisfies Eq. (\ref{eq:det-sample}) for a fixed set $A$ and $B$ of size at most $a$ and $b$ (respectively) is $q=p^a\cdot (1-p)^b=1/a^b$. The probability that none of the subgraph $G_i$ satisfy   Eq. (\ref{eq:det-sample}) for $A,B$ is at most $(1-q)^{a^{b+1}\cdot \log n}\leq 1/n^{3a}$. Thus, by doing a union bound over all $n^{2a}$ possible subsets of $A,B$, we get that $\mathcal{G}_R$ satisfies Eq. (\ref{eq:det-sample}) for all subsets with positive probability. The lemma follows.
\end{proof}
%}%\APPENDLEMPROB
Lemma \ref{lem:prob-approach-det-sample} already implies a deterministic minimum cut algorithm with $\poly(D)$ rounds, in case where nodes are allowed to perform \emph{unbounded} local computation. Specifically, let every node compute locally, in a brute force manner, the family of graphs $\mathcal{G}=\{G_i \subseteq G\}$ of size $a^{b+1}\cdot \log n$. In each iteration $i$ of the minimum-cut computation, nodes will use the graph $G_i \in \mathcal{G}$ to compute the truncated BFS tree, and collect their tree paths in these trees. Although the \congest\ model does allow for an unbounded local computation, it is still quite undesirable. To avoid this, we next describe an explicit \emph{polynomial} construction of the graph family $\mathcal{G}$. This explicit construction is based on stating our requirements in the language of universal sets. 

\dnsparagraph{Universal Sets} A family of sets $\mathcal{S}=\{S \subseteq [n]\}$ is $(n,k)$-\emph{universal} if every subset $S' \subseteq [n]$ of $|S'|=k$ elements is \emph{shattered} by $\mathcal{S}$. That is, for each of the $2^k$ subsets $S'' \subseteq S'$ there exists a set $S \in \mathcal{S}$ such that $S'\cap S=S''$. Using linear codes, one can compute $(n,k)$-universal sets with $n^{O(k)}$ subsets. Alon \cite{alon1986explicit} showed an explicit construction of size $2^{O(k^4)}\log n$ using the Justesen-type codes  constructed by Friedman \cite{friedman1984constructing}. 
In our context, the parameter $n$ corresponds to the number of graph edges, and each subset is a subgraph. The parameter $k$ corresponds to the bound on the length of the path which is $O(\lambda \cdot D)$. Using the existing constructions lead to a family with $2^{\lambda \cdot D}$ subgraphs which is unfortunately super-linear, already for graphs of logarithmic diameter. 

\dnsparagraph{A New Variant of Universal Sets} We define a more relaxed variant of universal sets, for which a considerably improved size bounds can be obtained. In particular, for our purposes it is not really needed to fully shatter subsets of size $k$. Instead, for every set $S'$ of $k$ elements we would like that for every small subset $S''\subseteq S$, $|S''|\leq b$ (which plays the role of the faulty edges),  there will be a set $S$ in the family satisfying that $S' \cap S=S'\setminus S''$. 
We call this variant FT-universal sets, formally defined as follows.
%
%In our context, we define a more specific universal sets, that allows us to obtain considerably better bounds on the cardinality of the set collection.  
%\begin{definition}[FT-Universal Sets]
%For integers $n,k,f$ where $f<k$, a family of sets $\mathcal{S}=\{ S \subset [1,n]\}$ is $(n,k,q)$-\emph{universal} if for every set $S' \subset [1,n]$, $|S'| \leq k$, and for every subset $S'' \subset S$ of cardinality at most $q$, there exists a set $S \in \mathcal{S}$ such that: (1) $S'' \cap S=\emptyset$ and (2) $S' \setminus S'' \subseteq S$. 
%\end{definition}
%\vspace{-7pt}
\begin{definition}[FT-Universal Sets]
For integers $n,a,b$ where $a\leq b \leq n$, a family of sets $\mathcal{S}=\{ S \subset [1,n]\}$ is $(n,a,b)$-\emph{universal} if for every two disjoint subsets $A \subset [1,n]$ and $B \subset [1,n]$ where $|A|\leq a$ and $|B|\leq b$, there exists a set $S \in \mathcal{S}$ such that (1) $A \subseteq S$ and (2) $B \cap S=\emptyset$.
%
%$S' \subset [1,n]$, $|S'| \leq k$, and for every subset $S'' \subset S$ of cardinality at most $q$, there exists a set $S \in \mathcal{S}$ such that: (1) $S'' \cap S=\emptyset$ and (2) $S' \setminus S'' \subseteq S$. 
\end{definition}\vspace{-3pt}
Our goal is compute a family of $(n,a,b)$-universal sets of cardinality $O(a^{b+1}\log n)$ in time $\poly(n,a^b)$. 
Towards that goal we will use the notion of perfect hash functions.
\begin{definition}[Perfect Hash Functions]
For integers $n$ and $k<n$ a family of hash functions $\mathcal{H}=\{h: [n] \to [\ell]\}$ is \emph{prefect} if for every subset $S \subset [1,n]$ for $|S| \leq k$, there exists a function $h \in  \mathcal{H}$ such that
$h(i) \neq h(j), ~~~\forall i, j \in S, i \neq j.$
\end{definition}
\vspace{-10pt}
\begin{definition}[Almost Pairwise Independence]\label{def:almost}
A family of functions $\mathcal{H}$ mapping domain $[n]$ to range $[m]$ is $\epsilon$-almost pairwise independent if for every $x_1 \neq x_2 \in [n]$, $y_1,y_2 \in [m]$, we have:
$\Pr[h(x_1)=y_1 \mbox{~and~} h(x_2)=y_2]\leq (1+\epsilon)/m^2.$
\end{definition}
%\vspace{-10pt}
\begin{fact}[\cite{TCS-010}]\label{fact:pihash}
For every $\alpha,\beta \in \mathbb{N}$ and $\epsilon \in (0,1)$, one can compute in $\poly(\alpha \cdot 2^{\beta}\cdot 1/\epsilon)$ an explicit family of $\epsilon$-almost pairwise independent hash functions $\mathcal{H}_{\alpha,\beta}=\{h: \{0,1\}^\alpha \to \{0,1\}^\beta\}$ that contains $O(\alpha \cdot 2^{\beta})$ functions. 
\end{fact}%\vspace{-7pt}
%\begin{fact}[Thm. 3.26 in \cite{TCS-010}]\label{fact:pihash}
%For every $a,b \in \mathbb{N}$, one can compute in $\poly(2^{a+b})$ an explicit family of pairwise independent hash functions $\mathcal{H}_{a,b}=\{h: \{0,1\}^a \to \{0,1\}^b\}$ that contains $2^{a+b}$ functions. 
%\end{fact}
We next show how to compute a family of $(n,k)$-perfect hash functions in polynomial time.
%\vspace{-4pt}
\begin{claim}\label{cl:small-perfect}
One can compute an family of $(n,k)$-perfect  hash functions $\mathcal{H}=\{h: [n] \to [2k^2]\}$ of cardinality $O(k^4 \log n)$ in time $\poly(n,k)$.
\end{claim}%\vspace{-7pt}
%\def\APPENDSMALLPERF{
\begin{proof}%[Proof of Claim \ref{cl:small-perfect}]
We use Fact \ref{fact:pihash} with $\alpha=\log n$, $\beta=4\log k$, and $\epsilon=0.1$, to get an $\epsilon$-almost pairwise independent hash function family $\mathcal{H}_{\alpha,\beta}=\{h: \{0,1\}^\alpha \to \{0,1\}^\beta\}$. 
We now show that this family is perfect for subsets $S \in [1,n]$ of cardinality at most $k$.
Fix a subset $S \in [1,n]$, $|S|\leq k$. By definition, for every $x_1, x_2 \in S$ and $y_1, y_2 \in [2k^2]$,
$$\Pr_{h \in \mathcal{H}}[h(x_1)=y_1 \mbox{~and~} h(x_2)=y_2]\leq (1+\epsilon)/(4 k^4).$$
Thus, the probability that a uniformly chosen random function $h \in \mathcal{H}_{a,b}$ collides on $S$ is 
\begin{eqnarray}
\sum_{x_1 \neq x_2 \in S}\Pr_{h \in \mathcal{H}}[h(x_1)=h(x_2)]&\leq& k^2 \cdot \max_{x_1 \neq x_2 \in S}\Pr_{h \in \mathcal{H}}[h(x_1)=h(x_2)]
\\& =& \nonumber
k^2\cdot \max_{x_1 \neq x_2 \in S}\sum_{y \in [2k^2]}\Pr[h(x_1)=h(x_2)=y]\leq 0.3~, \nonumber
\end{eqnarray}
by using the fact that $\Pr_{h \in \mathcal{H}}[h(x_1)=h(x_2)=y]\leq (1+\epsilon)/(4k^4)$ (
see Def. \ref{def:almost}). We get that there exists $h' \in \mathcal{H}_{\alpha,\beta}$ that has no collisions on $S$. As this holds for every $S$, the claim follows.
\end{proof}
%}%\APPENDSMALLPERF
%\APPENDSMALLPERF
Equipped with the polynomial construction of families of $(n,k)$-perfect hash functions, we next show how to compute our universal sets in polynomial time.
%\vspace{-7pt}
\begin{lemma}[Small Universal Sets]\label{lem:universalsets}
For every set of integers $b<a<n$, one can compute in $\poly(n,a^{b})$, a family of universal sets $\mathcal{S}_{n,a,b}$ of cardinality $O(a^{b+1} \cdot \log n)$.
\end{lemma}%\vspace{-7pt}
\begin{proof}
Set $k=a+b$. We will use Claim \ref{cl:small-perfect} to compute an $(n,k)$-perfect family of hash functions $\mathcal{H}=\{h: [n] \to [2k^2]\}$. 
For every $h \in \mathcal{H}$ and for every subset $i_1,\ldots, i_b \in [1,2k^2]$, define:
$$S_{h,i_1,i_2,\ldots, i_b}=\{ \ell \in [n] ~\mid~ h(\ell) \notin \{i_1,i_2,\ldots, i_b\}\}~.$$
Overall, $\mathcal{S}_{n,a,b}=\{S_{h,i_1,i_2,\ldots, i_b} ~\mid~ h \in \mathcal{H}, i_1,i_2,\ldots, i_b \in [1,2k^2]\}$. 

The size of $\mathcal{S}_{n,a,b}$ is bounded by $|\mathcal{H}|\cdot k^{2b}=O(k^{3b} \cdot \log n)$ as desired.
We now show that $\mathcal{S}_{n,a,b}$ is indeed a family of universal sets for $n,a,b$. 
Since $\mathcal{H}$ is an $(n,k)$ perfect family of hash functions, for every two disjoint subsets $A,B \subset [n]$, $|A|\leq a$ and $|B|\leq b$, there exists a function $h$ that does not collide on $C=A \cup B$ (since $|C|\leq k$). That is, there exists a function $h \in \mathcal{H}$ such that $h(i) \neq h(j)$ for every $i,j \in C$, $i \neq j$. 
Thus, letting $B=\{s_1,\ldots, s_b\}$ and $i_1=h(s_1),\ldots, i_b=h(s_b)$, we have that $h(s'_j)\notin \{i_1,\ldots, i_b\}$ for every $s'_j \in A$. Therefore, the subset $S_{h,i_1,i_2,\ldots, i_b}$ satisfies that 
$A  \subseteq S_{h,i_1,i_2,\ldots, i_b}$ and $B \cap  S_{h,i_1,i_2,\ldots, i_b}=\emptyset$. 
\end{proof}

%\begin{corollary}\label{cor:unisets}
%For every $n,k,q$, one can compute in $\poly(n,k,q)$, a family of universal sets of cardinality $k^{\poly(q)}$.
%\end{corollary}
\paragraph{Deterministic Min-Cut Algorithm.}
Finally, we describe how to use FT-universal sets to get a $\poly(D)$-round distributed algorithm for exact computation of small cuts. The only randomized part of the algorithm above is in defining the $\ell=\poly(D)$ subgraphs $G_i$. Instead of sampling these subgraphs, each vertex computes them explicitly and locally. First, we rename all the edges to be in $[1,m]$. This can be easily done in $O(D)$ rounds. 
Now, each vertex locally computes a family of universal sets for parameters $m,k=O(\lambda \cdot D),q=\lambda$.
By Lemma \ref{lem:universalsets}, the family $\mathcal{S}$ contains $(\lambda \cdot D)^{\lambda}=\poly(D)$ subsets in $[1,m]$. Each of the sets $S_i \in \mathcal{S}$ will be used as a subgraph $G_i$ in the $i^{th}$ iteration. 
That is, we iterate over all subsets (subgraphs) in $\mathcal{S}$. In iteration $i$, all vertices know the set $S_i$ and thus can locally decide which of their incident edges is in $G_i$.
The correctness now follows the exact same line as that of the randomized algorithm.
%\begin{claim}
%For every vertex $v$, and for every sequence of $\lambda$ faults $F \subseteq E$, if $s$ and $v$ are connected in $G \setminus F$, then there is a subset $S_i \in \mathcal{S}$ (which defines the graph $G_i$), that contains all edges on the $s$-$v$ shortest path in $G \setminus F$ and does not contain any of the edges in $F$. 
%\end{claim}
%\begin{proof}
%Since $\dist(s,v,G \setminus F)=O(\lambda D)$, and $|F|\leq \lambda$, by the definition of the universal set $\mathcal{S}$, there exists a subset $S_i$ that contains $\pi(s,v, G \setminus F)$ and does not contain $F$. 
%\end{proof}
%The round complexity follows by the bound of $\poly(D)$ on the size of the universal sets. 
%
\section{Computation of All Edge Connectivities}\vspace{-5pt}
\input{cycle-cover.tex}
%The computation of edge connectivities (Thm. \ref{thm:edge-conn}) is deferred to Appendix \ref{sec:edge-conn}. 
%
%
%

%We therefore here: 
%\begin{lemma}
%For every unweighted $D$-diameter $n$-vertex graph, one can test if the graph is $\lambda$ edge-connected in $\widetilde{O}((\lambda D)^{2\lambda})$ rounds.
%\end{lemma}

%
%
%
%\paragraph{Computation of Edge Connectivities}
%
%
%
%\paragraph{Computation of Vertex Connectivities}
%
%
%
%This gives the following algorithm for computing minimum cuts of constant size. 
%
%%
%%\paragraph{Connectivity Decomposition.}
%%Immediately gives $\lambda$-edge connected components using $O((\lambda \cdot D)^{\lambda}+\sqrt{n})=O(\poly(D)+\sqrt{n})$. This is simply by computing the connected components on the graph induced on edges with connectivity $\lambda$. 
%%

%\def\APPENDEDGECONN{
%\input{cycle-cover.tex}
%}

